Analyzing Chat Protocols of Novice Programmers Solving Introductory Programming Tasks with ChatGPT

Large Language Models (LLMs) have taken the world by storm, and students are assumed to use related tools at a great scale. In this research paper we aim to gain an understanding of how introductory programming students chat with LLMs and related tools, e.g., ChatGPT-3.5. To address this goal, computing students at a large German university were motivated to solve programming exercises with the assistance of ChatGPT as part of their weekly introductory course exercises. Then students (n=213) submitted their chat protocols (with 2335 prompts in sum) as data basis for this analysis. The data was analyzed w.r.t. the prompts, frequencies, the chats' progress, contents, and other use pattern, which revealed a great variety of interactions, both potentially supportive and concerning. Learning about students' interactions with ChatGPT will help inform and align teaching practices and instructions for future introductory programming courses in higher education.

==> methodology.tex <==
The "Introduction to Practical Computer Science" (German: "Einführung in die Praktische Informatik", EPI) module, offered at Goethe University, incorporates the "Introduction to Programming" (German: "Einführung in die Programmierung", EPR) course as a fundamental component. This course is designed to introduce students to the foundational principles of programming and is structured to unfold annually during the winter term. Spanning one semester, EPR aims to equip participants with the essential skills and knowledge required to navigate the field of computer science effectively.

EPR is conducted in German, ensuring that the course material is accessible and engaging for the target audience. The course format includes two hours of lecture per week, complemented by two-hour tutorial sessions in smaller groups of 20-30 students. These tutorials are integral to the learning process, providing a more personalized and interactive experience. Additionally, the course is supported by an online moodle platform, supplementing the students' learning journey with digital resources and facilitating remote engagement.

A distinctive feature of EPR is the provision of weekly or bi-weekly exercise sheets. These sheets contain programming tasks that are not only central to the course's hands-on approach but also contribute to the students' assessment through a points system. While submissions are primarily individual, the course design incorporates approximately two exceptions that allow for partner submissions, fostering collaboration among students.

Initially attracting 790 participants in winter term 2023/24, the course demographic is predominantly computer science students, although it also open to individuals from other majors who pursue computer science as a minor. Notably, EPR is accessible from the first semester onwards, with no prerequisites, making it a starting point for novices to the discipline.

\subsection{RQ1 Exercise Implementation and ChatGPT-3.5 Integration}

For the exploration of RQ1 within the context of the "Introduction to Programming" course, a specific methodology was employed regarding the exercise sheets. This methodological framework outlines the formalities associated with the distribution, completion, and submission of these exercise sheets, as well as the guidelines provided to students for utilizing ChatGPT-3.5.

\textit{Handout and Submission Process}. Exercise sheets were distributed and submitted through the established Moodle course platform, a procedure familiar to the students. This ensured a seamless integration into the existing course structure, minimizing confusion and maximizing accessibility.

\textit{Language Availability}. To accommodate a diverse student body, exercises were made available in both German and English, providing linguistic flexibility and ensuring that more students could engage with the material in their preferred language.

\textit{Submission Constraints}. Students were required to adhere to usual submission guidelines, including the provision of documentation (e.g., author name) and adherence to specified file formats for submissions, ensuring consistency and fairness in the evaluation process.

%shorten
%\textit{Plagiarism Policy Exception}. An exception was made to the usual plagiarism policy for this exercise, stating that no points would be deducted for plagiarism or insufficient original work. This adjustment was made to encourage experimentation with ChatGPT-3.5 without the fear of penalization.

\textit{Submission Timeline}. Students were given a two-week window to complete and submit their exercises, affording them ample time to engage with ChatGPT-3.5 and integrate its outputs into their work.

\textit{Submission and Tool Use Instructions}. Submissions were to be individual, and students were explicitly instructed to utilize the free version of ChatGPT-3.5 via its web interface\footnote{https://chat.openai.com/}. However, no specific instructions were provided on how to interact with ChatGPT-3.5 beyond a reference to OpenAI's guide on prompt engineering\footnote{https://platform.openai.com/docs/guides/prompt-engineering}. This approach was deliberately chosen to minimize bias by avoiding any influence over the students' methods of interacting with ChatGPT-3.5, ensuring that their use of the tool reflected their genuine approach and understanding..

\textit{Documentation and Participation Incentives}. Students were advised to document their interactions with ChatGPT-3.5 in a .xlsx format5, specifically recording both the prompts they provided and the corresponding answers, as paired entries. Participation in this aspect of the exercise was incentivized with extra points (2 out of 8), highlighting the value placed on engaging with ChatGPT-3.5. It was clarified that using ChatGPT was optional, with a significant portion of the points still obtainable through traditional problem-solving (6 out of 8).

\textit{Instructional Support}. The exercise and its research objectives were explained during a lecture session. This session included guidance on template usage for the exercise submission and addressed formal inquiries related to the exercise setup. Notably, content-specific questions that might influence the independent use of ChatGPT-3.5 were not discussed to ensure the integrity of the research.

This methodological approach was designed to facilitate an unbiased exploration of ChatGPT-3.5's potential as a supportive tool for programming novices, allowing for a naturalistic integration of the LLM into their learning process while maintaining the known structured educational environment of the course.

\subsubsection{Exercise Content}

The exercise content was designed around the topic of \textit{recursion}, in addition to the concepts of \textit{functions}, \textit{lists}, \textit{conditionals}, \textit{string manipulation}, and \textit{documentation}. The exercise comprised two main tasks.

\textit{The first task} was divided into four subtasks, each presenting a distinct code snippet employing recursion. This task design was similar to previous exercises and representing potential exam questions. The subtasks focused on the recursive implementation of several operations:

\begin{enumerate}[label=(\alph*)]
    \item Summing the digits of a number
    \item Reversing a list
    \item Performing multiplication
    \item The Ackermann function
\end{enumerate}

Students were not required to write code; instead, their task was to read and interpret these code snippets. Specifically, they were to determine the output of the code, the number of function calls made, and identify the type of recursion used.\\

\textit{The second task} presented a more complex challenge: implementing a function to determine the number of "happy strings" within all substrings of a given string. A "happy string" was defined as a string that can either be rearranged into (or already is) a repetition of some string twice. To solve this task, students were required to:

\begin{enumerate}
    \item Test a given string for the "happy" property
    \item Test all possible substrings of the given string
\end{enumerate}

While an iterative solution was possible, students were encouraged to adopt a recursive approach, with additional points awarded for recursive implementations.\\

\textit{Task Selection and Testing}. The tasks were selected and repeatedly tested to evaluate ChatGPT-3.5's capability to solve them. In task 1, ChatGPT demonstrated a high success rate in identifying the correct functions but frequently erred in calculating the number of calls, often overlooking the base case. Task 2 proved more challenging for ChatGPT; although it could outline the necessary steps for solving the problem, it struggled to deliver correct solutions, possibly due to the ambiguous wording of the task.\\

\subsubsection{Participant Engagement and Data Collection}

The template, designed to document prompt/response pairs, alongside the comprehensive survey, constituted the core methodological instruments for addressing RQ 1.
A total of 360 students successfully completed the exercise designed to explore the utilization of ChatGPT-3.5 in solving programming tasks. Of these, 305 students engaged with ChatGPT-3.5 as part of the exercise. However, due to the absence of the required template usage or submission in non-processable file formats, the data from 95 students could not be included in the final analysis. Consequently, the refined dataset comprised 213 students, providing a substantial collection of 2335 prompts for detailed examination. Additionally, 298 students participated in the survey, offering insights into their experiences and perceptions of using ChatGPT-3.5 for programming tasks.




\subsection{Data Analysis}

Following the data collection, the study progresses to the evaluation of the gathered data. This next step involves delineating and applying a set of defined evaluation parameters designed to systematically assess ChatGPT-3.5's responses in the context of the selected tasks and student submissions. 

Identify quantitative measures of prompt use, identify median of prompt use, 

We distinguish by number of prompts used by students, and analyze their patterns based on the use of prompts: 0-5 means that student usually used one prompt per subtask. 

We used ...



\subsection{RQ1 Evaluation Criteria for Prompt and Survey Analysis}

To address RQ1, this study employs a two-pronged approach, integrating both prompt analysis and survey data. Through the examination of prompts, the aim is to uncover the nuances of student interactions with ChatGPT-3.5, identifying patterns and trends in how programming novices seek assistance from the AI. 

This study employs a comprehensive set of evaluation parameters for analyzing the responses generated by ChatGPT-3.5 to each prompt. These parameters are designed to dissect the nuances of the interactions between the students and ChatGPT-3.5 to address RQ1.1.\\

\textbf{Prompt Analysis Parameters:}
\begin{itemize}
    \item \textit{Language}: The language used in the prompt (English, German and/or Code), recognizing the potential impact of linguistic nuances on the AI's response accuracy and relevance.
    \item \textit{Number of Prompts}: The total count of prompts given to ChatGPT-3.5, offering insights into the extent of interaction from students with the AI.
    \item \textit{Number of Words per Prompt}: This metric gauges the verbosity or conciseness of prompts, which may correlate with the clarity or complexity of the questions posed to ChatGPT-3.5.
    \item \textit{Follow-up Interactions}: Categorized based on whether a prompt is a standalone query, a follow-up to a previous prompt, a response to a ChatGPT answer, or a correction of a previous response. This parameter aims to capture the iterative nature of problem-solving interactions with ChatGPT-3.5.
    \item \textit{Category of Problem Solving}: This classification identifies the type of cognitive or programming task the prompt is addressing, including problem understanding, conceptual understanding, code generation, debugging, runtime analysis, syntax/style, documentation, test cases, and other categories.
    \item \textit{Solution Indication}: Determines whether the prompt explicitly seeks a direct solution, shedding light on the intention behind the query and the expected outcome of the interaction (e.g. only the task is prompted).
\end{itemize}



==> related_work.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Structured LLM Applications in Educational Frameworks}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Codehelp
% rw_sw_guided01

% 3
% et al. \cite{rw_sw_guided01} describe the development of CodeHelp, a web-based tool aimed at supporting programming students without directly revealing solutions. CodeHelp uses a multi-prompt LLM workflow designed to generate helpful responses while ensuring content relevance and avoiding complete solutions (p. 5 \cite{rw_sw_guided01}). The system also includes features for instructors, such as class configuration and monitoring of student interactions (p. 6 \cite{rw_sw_guided01}). The instructor noted CodeHelp's ease of introduction, its role in providing initial support for common issues, and its utility for students outside of office hours. Challenges included aligning CodeHelp's advice with course content and teaching students to provide detailed problem descriptions (p. 9-10 \cite{rw_sw_guided01}). A survey conducted at the semester's end showed high student appreciation for CodeHelp. Most students found it valuable for completing work and learning course material, expressing interest in using it in future courses (p. 8 \cite{rw_sw_guided01}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Experiences from Using Code Explanations
% rw_sw_guided02

% 4
%Stephen MacNeil et al. \cite{rw_sw_guided02} investigated the impact of code explanations generated by LLMs in a web software development e-book. The authors used prompt engineering to select the most effective LLM, the creation of different types of explanations (\enquote{line-by-line, summarization, and listing concepts}) for code snippets (p. 934 \cite{rw_sw_guided02}). Comparing explanations generated by GPT-3 and Codex, the authors concluded that GPT-3 produced better quality explanations. Codex's explanations often went off-topic or included irrelevant code snippets, whereas GPT-3 provided more useful and structured content (p. 935 \cite{rw_sw_guided02}).
% 6.2
%Engagement varied, with about half of the students who accessed the e-book engaging with the explanations. Curiosity and code complexity were primary drivers for engagement. The first code snippet and more complex later snippets saw higher engagement. This indicates that the format and content of the e-book itself, which had been effectively used for teaching before the introduction of LLM-generated explanations, might have influenced the engagement levels. The additional explanations provided by LLMs did not significantly alter how students used the e-book (p. 935 \cite{rw_sw_guided02}).
% 6.3
%Preliminary findings suggest that explanations were helpful for learning, with students rating them as relevant and useful. Despite line-by-line explanations being the most requested, students rated summary explanations as more helpful for learning. The correct but sometimes overly detailed or incorrectly focused nature of some explanations was noted, suggesting room for improvement in prompt engineering and explanation generation methods (p. 935 \cite{rw_sw_guided02}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GPTutor
% rw_sw_guided03
%The paper from Eason Chen et al. \cite{rw_sw_guided03} introduces \enquote{GPTutor}, a ChatGPT-powered Visual Studio Code extension designed to enhance programming education by providing personalized code explanations. GPTutor leverages ChatGPT API to analyze and explain code directly within the editor, intending to offer a more efficient learning tool compared to existing methods like vanilla ChatGPT and GitHub Copilot. It is indicated to be user-friendly and effective in delivering concise and accurate explanations (p. 5 \cite{rw_sw_guided03}). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Repairing Bugs in Python
% rw_sw_guided04

% IV
%Jialu Zhang et al. \cite{rw_sw_guided04} introduce a \enquote{multi-modal automated repair system} (MMAPR) architecture, designed for repairing syntax and semantic errors in Python programming assignments. It describes a two-phase approach: syntax repair and semantic repair. The syntax phase identifies and corrects syntax errors using chunking and \enquote{syntax-oriented prompts}. The semantic phase addresses semantic errors, employing \enquote{semantic prompts} that may include few-shots from similar student submissions (p. 4-6 \cite{rw_sw_guided04}). 
% V-A
%The results highlight the effectiveness of the system in identifying and correcting both syntax and semantic errors, showing a improvement in repair accuracy compared to baseline approaches (p. 7 \cite{rw_sw_guided04}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Using LLMs to Enhance Error Messages
% rw_sw_guided05

% 3.2
%Juho Leinonen et al. \cite{rw_sw_guided05} focuses on the generation of enhanced programming error messages using the latest Codex model. It explores prompt engineering to evaluate different types of prompts for their effectiveness in generating useful explanations. Five distinct prompt styles were tested to determine which produced the fewest empty responses from Codex, with the goal of finding the most effective prompt for generating understandable and actionable error explanations (p. 564-565 \cite{rw_sw_guided05}).
% 4
%The results show a improvement in the clarity and usefulness of error messages, suggesting that Codex can effectively assist programmers in debugging by providing more insightful explanations than traditional compiler errors (p. 566 \cite{rw_sw_guided05}). It is suggested that clearer, more informative error messages could notably benefit novice programmers by reducing frustration and learning barriers (p. 567 \cite{rw_sw_guided05}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%Studying the effect of AI Code Generators

% 3
%The work of Majeed Kazemitabaar et al. \cite{rw_sw_05} describes the creation and utilization of "Coding Steps," a web-based application designed to teach basic Python programming through a series of progressively complex tasks. This environment integrates various features like a code editor with syntax highlighting, real-time error detection, Python documentation tailored for novices, and an AI code generator powered by OpenAI Codex (p. 3-5 \cite{rw_sw_05}).
% 4
%The study aimed to evaluate the effectiveness of AI code generators in supporting beginners by observing their interaction with the tool, their progress in programming tasks, and their overall learning experience (p. 6-7 \cite{rw_sw_05}). 
% 5
%It shows positive outcomes in terms of improved understanding of programming concepts, increased confidence in coding, and enhanced problem-solving skills. The results indicate that the AI code generator supports novice learners by providing real-time assistance and personalized feedback, thereby facilitating a more effective and engaging learning experience (p. 11-12 \cite{rw_sw_05}).\\
%
%From examining the role of LLMs within structured educational frameworks, the discussion progresses to the exploration of LLMs in self-directed learning environments. This progression underscores the adaptability of LLMs to support autonomous student engagement, where learners harness these tools to solve problems independently.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{LLMs in self directed Learning Environments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%Exploring LLM to Generate Formative Feedback
% rw_sw_01

%The paper from Kiesler et al. \cite{rw_sw_01} explores the use of ChatGPT from the students' perspective by evaluating its effectiveness in providing formative feedback on programming assignments. It examines ChatGPT's responses to incorrect student submissions in introductory programming tasks, focusing on the content, quality, and types of feedback generated (p. 3 \cite{rw_sw_01}). The study highlights ChatGPT's capability to detect and correct compile errors, offering \enquote{textual explanations of errors and fixes with improved code} (p. 5 \cite{rw_sw_01}). Nevertheless, there are limitations in \enquote{feedback quality on logic and semantic errors}, as well as misleading information (p. 5 \cite{rw_sw_01}). 

%\cite{azaiz2024feedbackgeneration}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%Exploring the Responses of LLM
% rw_sw_02

%The work of Hellas et al. \cite{rw_sw_02} assesses the potential of LLMs, specifically OpenAI Codex and GPT-3.5, to support novice programmers by analyzing their responses to actual help requests from an online programming course. By selecting a diverse range of requests, the study aims to cover a wide spectrum of common programming issues encountered by beginners (p. 3-4 \cite{rw_sw_02}).
%The findings suggest that, although LLMs demonstrate potential in identifying and addressing some types of programming queries, there are notable limitations in their responses, indicating a need for further refinement and customization for educational use (p. 6-7 \cite{rw_sw_02}).

%The work underscores the potential of LLMs in educational contexts, while also highlighting the challenges in ensuring the feedback is pedagogically valuable and comprehensible to novices. The authors call for further research into optimizing LLMs for educational purposes and suggest that future developments could significantly enhance programming education by providing tailored feedback to students (p. 11 \cite{rw_sw_02}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%Exploring the Use of ChatGPT as Tool
% rw_sw_03

%Basit Qureshi \cite{rw_sw_03} investigates the impact of ChatGPT in an educational setting, focusing on programming challenges within a computer science course at Prince Sultan University. It contrasts the performance of two student groups in a Data Structures and Algorithms course: one using traditional study materials and the other utilizing ChatGPT (p. 4 \cite{rw_sw_03}). The findings reveal that students using ChatGPT scored higher, though not without facing issues like code inaccuracies and inconsistencies. (p. 5-6 \cite{rw_sw_03})
%This study highlights the potential benefits of integrating AI tools like ChatGPT in education, including enhanced student engagement and learning outcomes, while also cautioning against possible pitfalls such as over-reliance on AI for problem-solving and risks to academic integrity (p. 7 \cite{rw_sw_03}).

